A Divide et Impera Approach for 3D Shape Reconstruction from Multiple Views

Estimating the 3D shape of an object from a single or multiple images has gained popularity thanks to the recent breakthroughs powered by deep learning. Most approaches regress the full object shape in a canonical pose, possibly extrapolating the occluded parts based on the learned priors. However, their viewpoint invariant technique often discards the unique structures visible from the input images. In contrast, this paper proposes to rely on viewpoint variant reconstructions by merging the visible information from the given views. Our approach is divided into three steps. Starting from the sparse views of the object, we first align them into a common coordinate system by estimating the relative pose between all the pairs. Then, inspired by the traditional voxel carving, we generate an occupancy grid of the object taken from the silhouette on the images and their relative poses. Finally, we refine the initial reconstruction to build a clean 3D model which preserves the details from each viewpoint. To validate the proposed method, we perform a comprehensive evaluation on the ShapeNet reference benchmark in terms of relative pose estimation and 3D shape reconstruction.

==> results/shape_estimation_chamfer.tex <==
\begin{table}
    %\resizebox{\columnwidth}{!}{
      \centering
       \setlength{\tabcolsep}{1.5mm}
      {\small
      \begin{tabular}{l|ccccccccc|ccc}
      \toprule
      Method &\multicolumn{3}{c}{Airplane} & \multicolumn{3}{c}{Car}  & \multicolumn{3}{c}{Chair} & \multicolumn{3}{|c}{Mean} \\
      \midrule
      3D-R2N2 \cite{choy20163d}
      & 2.12 & 1.65 & 3.77 & 1.51 & 2.07 & 3.58 & 2.28 & 1.93 & 4.21 & 1.97 & 1.89 & 3.86 \\
      Pix2Vox \cite{Xie_2019_ICCV}
      & 1.57 & 1.62 & 3.20 & 1.47 & 2.07 & 3.54 & 1.73 & 2.04 & 3.77 & 1.59 & 1.91 & 3.50 \\
      Ours Canonical View 
      & 1.46 & 1.47 & 2.92 & 1.47 & 2.05 & 3.51 & 1.48 & 1.92 & 3.39 & 1.47 & 1.81 & 3.28 \\
      Ours GT poses                  
      & 1.87 & 1.98 & 3.85 & 1.73 & 1.90 & 3.63 & 1.92 & 2.14 & 4.06 & 1.84 & 2.01 & 3.85 \\
      Ours optimized poses           
      & 2.31 & 2.50 & 4.81 & 1.90 & 2.03 & 3.93 & 2.24 & 2.51 & 4.75 & 2.15 & 2.34 & 4.50\\
      \bottomrule
      \end{tabular}
      }
    %}
%   \vspace{3mm}
  \caption{\label{tab:shape_estimation_quant} Evaluation of shape prediction. We report the Chamfer distance between normalized point clouds multiplied by 100.}
\end{table}

==> results/shape_estimation_iou.tex <==
\begin{table}
    %\resizebox{\columnwidth}{!}{
      \centering
       \setlength{\tabcolsep}{1.5mm}
      {\small
      \begin{tabular}{l|ccc|c}
      \toprule
      Method & Airplane & Car  & Chair  & Mean \\
      \midrule
      3D-R2N2 \cite{choy20163d}      & 0.585            & 0.851             & 0.575             & 0.670 \\
      Pix2Vox \cite{Xie_2019_ICCV}   & 0.723            & \textbf{0.876}    & 0.612             & 0.737 \\
      Ours Canonical View            & \textbf{0.732}   & 0.874             & \textbf{0.648}    & \textbf{0.751} \\
      Ours GT poses & 0.654 & 0.659 & 0.592 & 0.635 \\    
      Ours optimized poses & 0.538 & 0.627 & 0.510 & 0.559 \\
      \bottomrule
      \end{tabular}
      }
    %}
  %\vspace{3mm}
  \label{tab:shape_estimation_iou}
  \caption{Intersection over union.}
\end{table}


